Evolving Generalizable Multigrid-Based Helmholtz Preconditioners with Grammar-Guided Genetic Programming

Solving the indefinite Helmholtz equation is not only crucial for the understanding of many physical phenomena but also represents an outstandingly-difficult benchmark problem for the successful application of numerical methods. Here we introduce a new approach for evolving efficient preconditioned iterative solvers for Helmholtz problems with multi-objective grammar-guided genetic programming. Our approach is based on a novel context-free grammar, which enables the construction of multigrid preconditioners that employ a tailored sequence of operations on each discretization level. To find solvers that generalize well over the given domain, we propose a custom method of successive problem difficulty adaption, in which we evaluate a preconditioner's efficiency on increasingly ill-conditioned problem instances. We demonstrate our approach's effectiveness by evolving multigrid-based preconditioners for a two-dimensional indefinite Helmholtz problem that outperform several human-designed methods for different wavenumbers up to systems of linear equations with more than a million unknowns.

==> src/helmholtz_equation.tex <==
Discretizing the two-dimensional Helmholtz equation with finite differences and a uniform grid with step size $h$ yields the linear system
\begin{equation}
	A_h u_h = f_h,
	\label{eq:discretized-system}
\end{equation}
where within the domain $A_h$ is represented by the five-point stencil
\begin{equation}
	A_h = \frac{1}{h^2} \begin{bmatrix}
		& -1 & \\
		-1 & 4 - (k h)^2 & -1 \\
		& -1 &  
	\end{bmatrix}.\label{eq:helmholtz-operator}
\end{equation}
For sufficiently large values of $k$, the matrix $A_h$ becomes indefinite, which imposes significant challenges on designing an efficient numerical solution method for this system.
The number of unknowns $N$ of the linear system~\eqref{eq:discretized-system} is given by $N = (1/h - 1)^2$, which means that the application of direct solution methods, such as Gaussian elimination, becomes infeasible for a sufficiently small step size $h$. 
As a remedy, iterative methods can be used to obtain an approximate solution in a finite number of steps.
%Basic iterative methods, such as the Jacobi and Gauss-Seidel method, suffer from slow convergence, and hence, more advanced techniques like Krylov subspace and multigrid methods are usually needed.
Unfortunately, many of these methods either require the matrix $A_h$ to be positive-definite or suffer from extremely slow convergence and, hence, can not be applied to Helmholtz problems with larger wavenumbers~\cite{ernst2012difficult}. 
Therefore, several approaches have been proposed to design an efficient iterative method for overcoming this difficulty, of which many are based on the idea of preconditioning the original system with one that is easier to solve, i.e., a system of the form of Equation~\eqref{eq:preconditioning-system}.
As Equation~\eqref{eq:helmholtz-preconditioned} illustrates, the preconditioned system is then solved up to the required accuracy, for instance, using a Krylov subspace method~\cite{saad2003iterative}.
Consequently, the task of constructing an efficient numerical method for solving the indefinite Helmholtz equation is reduced to two more manageable subproblems.
First, the system matrix $M$ must be chosen in a way that makes the resulting linear system efficiently solvable while at the same time effectively facilitate the solution of Equation~\eqref{eq:helmholtz-preconditioned}.
Second, since Equation~\eqref{eq:preconditioning-system} needs to be solved in every step of the preconditioned iterative method, an efficient algorithm is needed to approximate its solution with reasonably little computational effort. 
Due to their $h$-independent convergence, multigrid methods are a natural choice for this task.
An idea first proposed in \cite{erlangga2004preconditioner}  is the choice of the preconditioner $M$ as a complex-shifted version of $A$, such that
\begin{equation}
	M = -\nabla ^{2} - (k^{2} + \varepsilon i).
\end{equation}
A discretization with finite differences on a uniform grid then yields a five-point stencil of the form
\begin{equation}
	M_h = \frac{1}{h^2} \begin{bmatrix}
		& -1 & \\
		-1 & 4 - (k^2 + \varepsilon i) h^2 & -1 \\
		& -1 &  
	\end{bmatrix}.\label{eq:shifted-helmholtz-operator}
\end{equation}
In \cite{cocquet2017shift} it is shown that the choice of $\varepsilon$ represents a compromise between the resulting system's solvability and the effectiveness of the preconditioner.
In general, choosing the shift as $\varepsilon = \mathcal O(k^2)$ enables the effective approximate inversion of $M_h$ by multigrid, while lower values of $\varepsilon$ impede this task but lead to a more effective preconditioner.
While the choice of $\varepsilon$ represents an important decision in the preconditioner design, constructing an efficient multigrid method for the approximate inversion of the preconditioning matrix $M_h$ is of equal importance.
Unfortunately, in contrast to the choice of $M_h$, which boils down to a single parameter $\varepsilon$, the latter can be considered a problem of optimal algorithm design.
As presented in~\cite{schmitt2021evostencils,schmitt2020constructing} the rules for constructing a multigrid cycle can be specified in the form of a context-free grammar.

